Structural characterization of the interfacial self-assembly of chitosan with oppositely charged surfactant

Controlling the assembly of polyelectrolytes and surfactant at liquid-liquid interfaces offers new ways to fabricate soft materials with specific physical properties. However, little is known of the relationships between the kinetics of interfacial assembly, structural and rheological properties of such interfaces. We studied the kinetics at water-oil interface of the assembly of a positively charged biopolymer, chitosan, with an anionic fatty acid using a multi-scale approach. The growth kinetics of the membrane was followed by interfacial rheometry and space- and time- resolved dynamic light scattering. This set of techniques revealed that the interfacial complexation was a multi-step process. At short time-scale, the interface was fluid and made of heterogeneous patches. At a 'gelation' time, the surface elastic modulus and the correlation between speckles increased sharply meaning that the patches percolated. Confocal and electron microscopy confirmed this picture, and revealed that the basic brick of the membrane was sub-micrometric aggregates of chitosan / fatty acid.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
